Uoc luong kenh truyen trong he thong da robot su dung SDR

This study focuses on developing an experimental system for estimating communication channels in a multi-robot mobile system using software-defined radio (SDR) devices. The system consists of two mobile robots programmed for two scenarios: one where the robot remains stationary and another where it follows a predefined trajectory. Communication within the system is conducted through orthogonal frequency-division multiplexing (OFDM) to mitigate the effects of multipath propagation in indoor environments. The system's performance is evaluated using the bit error rate (BER). Connections related to robot motion and communication are implemented using Raspberry Pi 3 and BladeRF x115, respectively. The least squares (LS) technique is employed to estimate the channel with a bit error rate of approximately 10^(-2).

==> vncaps.tex <==
% Copyright 2000-2006 Werner Lemberg <wl@gnu.org> and
%                     Han The Thanh <hanthethanh@gmx.net>.
% This file is part of vntex.  License: LPPL, version 1.3 or newer,
% according to http://www.latex-project.org/lppl.txt

\ifx\ProvidesFile\undefined \else
  \ProvidesFile{vncaps.tex}[2006/06/07 v1.1 Captions in Vietnamese]  
\fi
 
% Vietnamese captions; edit them in viscii/tcvn/utf8, then use
% `vntovn viscii vntex' or a similar command to convert to vntex.
%
% History
%
% ????/??/??:
%     Split off captions from vietnam.ldf.
%     Add \captionsenglish, \dateUSenglish, and \dateenglish.
%
% 2005/04/21:
%     Add copyright message.
%     Don't use `{}' but a space after macros which don't have arguments.
%
% 2006/06/07:
%     Fix bug in \indexname.  Add version number.

\ifx\providecommand \undefined
  \let\providecommand \def
\fi

\providecommand\captionsvietnam{% 
  \def\prefacename{L\`\ohorn i n\'oi \dj\`\acircumflex u}%
%  \def\refname{T\`ai li\d\ecircumflex u}%
  \def\Acknowledgmentname{L\`\ohorn i c\h{a}m \ohorn n}%
  \def\refname{T\`ai li\d\ecircumflex u tham kh\h{a}o}%
%  \def\abstractname{T\'om t\'\abreve t n\d\ocircumflex i dung}
  \def\abstractname{T\'om t\'\abreve t}
  \def\IEEEkeywordsname{T\`\uhorn \, kh\'oa}
  \def\bibname{T\`ai li\d\ecircumflex u tham kh\h{a}o}%
  \def\chaptername{Ch\uhorn \ohorn ng}%
  \def\appendixname{Ph\d{u} l\d{u}c}%
  \def\contentsname{M\d{u}c l\d{u}c}%
  \def\listfigurename{Danh s\'ach h\`inh v\~e}%
  \def\listtablename{Danh s\'ach b\h{a}ng}%
  \def\indexname{Ch\h{i} m\d{u}c}% 
  \def\figurename{H\`inh}%
  \def\tablename{B\h{a}ng}%
  \def\partname{Ph\`\acircumflex n}%
  \def\pagename{Trang}%
  \def\headpagename{Trang}%
  \def\seename{Xem}%
  \def\alsoname{Xem th\ecircumflex m}%
  \def\enclname{K\`em theo}%
  \def\ccname{C\`ung g\h\uhorn i}%
  \def\headtoname{G\h\uhorn i}%
  \def\proofname{Ch\'\uhorn ng minh}}

\providecommand\datevietnam{%
  \def\today{%
    Ng\`ay \number\day\space
    th\'ang \number\month\space
    n\abreve m \number\year}}

\providecommand\captionsenglish{%
  \def\prefacename{Preface}%
  \def\refname{References}%
  \def\abstractname{Abstract}%
  \def\bibname{Bibliography}%
  \def\chaptername{Chapter}%
  \def\appendixname{Appendix}%
  \def\contentsname{Contents}%
  \def\listfigurename{List of Figures}%
  \def\listtablename{List of Tables}%
  \def\indexname{Index}%
  \def\figurename{Figure}%
  \def\tablename{Table}%
  \def\partname{Part}%
  \def\enclname{encl}%
  \def\ccname{cc}%
  \def\headtoname{To}%
  \def\pagename{Page}%
  \def\headpagename{Page}%
  \def\prefacename{Preface}%
  \def\seename{see}%
  \def\alsoname{see also}}

\providecommand\dateenglish{%
  \def\today{%
    \ifcase\day\or 1st\or 2nd\or 3rd\or 4th\or 5th\or 6th\or 7th\or
    8th\or 9th\or 10th\or 11th\or 12th\or 13th\or 14th\or 15th\or
    16th\or 17th\or 18th\or 19th\or 20th\or 21st\or 22nd\or 23rd\or
    24th\or 25th\or 26th\or 27th\or 28th\or 29th\or 30th\or 31st\fi
    ~\ifcase\month\or January\or February\or March\or April\or May\or
    June\or July\or August\or September\or October\or November\or
    December\fi \space
    \number\year}}

\providecommand\dateUSenglish{%
  \def\today{%
    \ifcase\month\or January\or February\or March\or April\or May\or
    June\or July\or August\or September\or October\or November\or
    December\fi \space\number\day, \number\year}}

\endinput

% end of vncaps.tex

